Revelation Gap for Pricing from Samples

This paper considers prior-independent mechanism design, in which a single mechanism is designed to achieve approximately optimal performance on every prior distribution from a given class. Most results in this literature focus on mechanisms with truthtelling equilibria, a.k.a., truthful mechanisms. Feng and Hartline (2018) introduce the revelation gap to quantify the loss of the restriction to truthful mechanisms. We solve a main open question left in Feng and Hartline (2018); namely, we identify a non-trivial revelation gap for revenue maximization. Our analysis focuses on the canonical problem of selling a single item to a single agent with only access to a single sample from the agent's valuation distribution. We identify the sample-bid mechanism (a simple non-truthful mechanism) and upper-bound its prior-independent approximation ratio by 1.835 (resp. 1.296) for regular (resp. MHR) distributions. We further prove that no truthful mechanism can achieve prior-independent approximation ratio better than 1.957 (resp. 1.543) for regular (resp. MHR) distributions. Thus, a non-trivial revelation gap is shown as the sample-bid mechanism outperforms the optimal prior-independent truthful mechanism. On the hardness side, we prove that no (possibly non-truthful) mechanism can achieve prior-independent approximation ratio better than 1.073 even for uniform distributions.

==> Figure/old/regular-large-opt-bid-rev2.tex <==
\begin{tikzpicture}[scale = 0.55]



\draw [white] (0, 0) -- (11.5, 0);
\draw (0,0) -- (10.5, 0);
\draw (0, 0) -- (0, 5.5);


\draw [dotted] (0, 5) -- (6.8, 5);
\draw (-0.3, 5) node {$1$};

\draw [line width=2.5pt, color=white!70!black] plot [smooth, tension=0.6] coordinates {
(0, 1) (3, 4) (6.8,5) 
};

\draw [line width=2.5pt, color=white!70!black] (6.8, 5) --(10,0);

\draw [line width=1.pt] plot [smooth, tension=0.6] coordinates {
(0, 1) (3, 4) (6.8,5) 
};

\draw [line width=1.pt] plot [smooth, tension=0.6] coordinates {
 (6.8,5) (8, 4.5) (9, 3) (10, 0)
};


\draw (0, -0.5) node {$0$};
\draw (10, -0.5) node {$1$};

\draw (6.8, -0.5) node {$\monoq$};
\draw [dotted] (6.8, 0) -- (6.8, 5);
\draw (6.8, 0) -- (6.8, 0.2);

\draw [dashed] (0, 0) -- (8, 5.882352941176471);
\draw (8.2, 6.3) node {$\monop$};
\draw [dashed] (0, 0) -- (10, 5.);
\draw (10.3, 5.3823) node {$\bid\primed$};

\draw (10, 3) node {$\rev_1$};
\draw (8, 1.5) node {$\rev_2$};

\end{tikzpicture}




==> Figure/old/regular-large-opt-bid-rev3.tex <==
\begin{tikzpicture}[scale = 0.55]

\draw [white] (0, 0) -- (11.5, 0);
\draw (0,0) -- (10.5, 0);
\draw (0, 0) -- (0, 5.5);


\draw [dotted] (0, 5) -- (6.8, 5);
\draw (-0.3, 5) node {$1$};

\draw [line width=2.5pt, color=white!70!black] plot [smooth, tension=0.6] coordinates {
(0, 1) (1, 2.162) 
};

\draw [line width=2.5pt, color=white!70!black] (1, 2.162) --(6.8,5);

\draw [line width=2.5pt, color=white!70!black] (6.8, 5) --(10,0);

\draw [line width=1.pt] plot [smooth, tension=0.6] coordinates {
(0, 1) (3, 4) (6.8,5) 
};

\draw [line width=1.pt] plot [smooth, tension=0.6] coordinates {
 (6.8,5) (8, 4.5) (9, 3) (10, 0)
};


\draw (0, -0.5) node {$0$};
\draw (10, -0.5) node {$1$};

\draw (6.8, -0.5) node {$\monoq$};
\draw [dotted] (6.8, 0) -- (6.8, 5);
\draw (6.8, 0) -- (6.8, 0.2);

\draw (1, -0.5) node {$\quant\doubleprimed$};
\draw [dotted] (1, 0) -- (1, 2.162);
\draw (1, 0) -- (1, 0.2);


\draw [dashed] (0, 0) -- (2.5, 5.404999999999999);
\draw (2.8, 5.8) node {$\bid\doubleprimed$};
\draw [dashed] (0, 0) -- (10, 5.);
\draw (10.3, 5.3823) node {$\bid\primed$};

\draw (10, 3) node {$\rev_1$};
\draw (8, 1.5) node {$\rev_3$};

\end{tikzpicture}




==> Paper/intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

% \YF{Revelation principle and 
% non-revelation mechanisms in practice}
Revelation principle, 
a seminal observation in mechanism design suggests that
if there is a mechanism with good equilibrium outcome,
there is a mechanism which
achieves the same outcome 
in a truthtelling equilibrium.
This constructed mechanism asks agents to report true
preferences,
simulates the agent strategies in the 
original mechanism, 
and outputs the outcome of the simulation.
Due to this guiding principle, 
a vast number of studies in mechanism design 
focus on revelation mechanisms 
(i.e., ones where revealing preferences truthfully forms
an equilibria).
However, successful applications
--
e.g., first-price auction, 
generalized second-price auction 
for advertisers in sponsored search
--
show
great practical impact of non-revelation 
mechanisms.
This motivates the research for understanding 
the
potential 
inadequacy of revelation principle
and 
advantages of non-revelation mechanisms
from a theoretical perspective.



% \YF{Prior-independent mechanism design,
% revelation gap, 
% open question for revelation gap in revenue}
To tackle this research motivation,
our paper lies in a line of research known as
prior-independent mechanism
design,
which
% In prior-independent mechanism design, 
% it 
considers Bayesian agents whose 
preference are drawn from a distribution (aka.\ prior)
that is unknown to the mechanism designer. 
The goal is to identify mechanisms
with good (multiplicative) prior-independent approximation
to the optimal mechanism
that is tailored to the distribution of preferences. 
In prior-independent mechanism design,
it is not generally without loss
to restrict to revelation mechanisms
--
the equilibrium strategies for Bayesian agents in 
non-revelation mechanisms are a function of 
their prior and thus the construction
of revelation mechanism
via revelation principle is no longer prior-independent.
Nonetheless, due to tractability and some other concerns, 
most results in prior-independent mechanism design
focus on revelation mechanisms.
To understand the loss of the restriction to revelation mechanisms,
\citet{FH-18} introduce revelation gap,
a quantification of optimal prior-independent approximation factor among
all revelation mechanisms vs.\ 
the optimal prior-independent approximation factor among all (possibly non-revelation)
mechanisms.
They identify a non-trivial revelation gap for
welfare-maximization
in a canonical model where agents are symmetric and have a common
budget constraint.
A main open question left in \citet{FH-18}
--
identifying a non-trivial revelation gap for revenue-maximization
--
embraces the following two challenges.

% \YF{Main difficult for revenue revelation gap:
% choice of model (avoid results from implementation theory),
% accurate analysis for non-revelation mechanism.}

% \YF{Single-agent revenue maximization with sample,
% revenue curve technique}

Given that the initial motivation is to 
provide theoretical justification for non-revelation mechanisms 
in practice, identifying the revelation gap  
needs to be asked with care.
The literature on non-parametric implementation theory
\citep[see the survey of][]{jac-01} suggests that,
in some canonical models
(e.g.\ single-item auction
for multiple symmetric agents),
the ``virtual implementations'' --
a sequential mechanism 
where agents interact in multiple rounds,
make reports about their own preferences 
and crossreport about their beliefs on other agents’ preferences
--
achieves
prior-independent approximation factor 
arbitrarily close one.
Such approaches from implementation theory 
contradict our initial motivation, 
since they 
take the model of Bayes-Nash equilibrium too literally 
and the resulting cross-reporting mechanisms are both fragile and impractical.
To overcome this issue,
in this paper, we consider a canonical model 
(i.e.\ single-item auction for single-agent with single-sample access,
see next paragraph)
and a simple non-revelation mechanism (i.e.\ \bidmech,
see more discussion in the next subsection)
that has also been studied in the economic literature 
for other purposes.

In mechanism design for single-item with single-agent,
under the standard regularity assumption on
the distribution of preference (aka.\ prior),
\citet{mye-81} and \citet{RZ-83} shows that the prior-dependent 
revenue-optimal mechanism 
is to post a take-it-or-leave-it price
depending on the 
prior.
It is not hard to see that the optimal prior-independent approximation
ratio among all mechanisms is infinite. 
Therefore, literature considers a modified model where 
mechanisms can access a single sample from the same distribution 
of agent's preference. 
\citet{DRY-15} show that posting this sample as the 
take-it-or-leave-it price achieves prior-independent approximation
factor 2 under the same regularity assumption.
\citet{AB-19} generalize this result
where they consider the class of sample-based pricing 
--
posting the sample with a (possibly randomized) scalar as the 
take-it-or-leave-it price,
and give both upper bound and lower bound of 
the optimal prior-independent approximation factor among 
all mechanisms in this class.
In this paper, we consider the same model as \citet{DRY-15}
and \citet{AB-19}.
We design a simple non-revelation mechanism and show that
its prior-independent approximation factor is strictly 
better than that of the best revelation mechanism.\footnote{We impose a technical assumption
(i.e.\ scale-invariant)
to the class of revelation mechanisms,
which is common in prior-independent mechanism
design \citep{AB-18,AB-19,HJL-19}.}
We also give a lower bound of optimal prior-independent 
approximation factor among all mechanisms,
indicating the nonexistence of the ``virtual implementations''
from the non-parametric implementation theory in this setting.

The second challenge for identifying a revelation gap 
is the requirement of precise prior-independent approximation 
analysis for non-revelation mechanisms. 
Though much of the theory in mechanism design is developed for revelation mechanisms,
there are some techniques (e.g.\ price of anarchy) to analyze the approximation guarantee 
for non-revelation mechanisms in the literature.
However, most of those results and techniques are 
problem or mechanism specific and 
only leads to relatively loose
approximation guarantees.
They are insufficient to 
prove the outperformance of the prior-independent approximation ratio
from a given non-revelation mechanism 
against that of the best revelation mechanism.\footnote{In \citet{FH-18},
authors bypass this challenge by considering symmetric environment where the all-pay auction \citep[cf.][]{mas-00} 
achieves prior-independent approximation factor 1,
i.e., it is indeed Bayesian optimal mechanism.
}
On the other side, for the class of revelation mechanisms,
there are general techniques which provide precise or even tight 
approximation guarantee.
One of such successful technique is  
the 
revenue curves analysis, 
% \citep[cf.][]{BR-89},
which has been used extensively in prior-independent 
mechanism design \citep[e.g.][]{DRY-15, AB-18,AB-19,HJL-19}
and other other lines of research 
\citep[e.g. simple vs.\ optimal --][]{AHNPY-18,JLTX-19,JLQTX-19,FHL-19,FHL-20}.
In this paper, thanks to the simplicity of
our proposed non-revelation mechanism,
we adapt the revenue curve analysis for its approximation 
guarantee.
See more discussion of the revenue curve analysis 
% for non-revelation mechanisms 
in the next subsection.


\subsection*{Main Results}
In this paper, we identify a non-trivial
revelation gap for revenue-maximization.
This theorem follows from three results.
First, we introduce 
the \bidmech\
(defined below) and obtain 
an upper bound of 
its prior-independent approximation factor
based on an analysis on revenue curves.
Second, we obtain a lower bound of the
optimal prior-independent approximation factor 
among all possible mechanisms.
Third, we show any revelation mechanism  
is equivalent to a sampled-based pricing mechanism
(defined below) introduced by 
\citet{AB-19} 
where authors
lower-bound
and upper bound the optimal
prior-independent approximation factor 
among all sample-based pricing.
Since the prior-independent approximation factor of the \bidmech\ 
is strictly better than 
the optimal prior-independent approximation factor 
among all revelation mechanisms, we 
immediately get our non-trivial revelation gap for 
revenue-maximization.
See \Cref{tab:summary} for a summary of all three results.

In the model of 
single-agent with single-sample access, 
the class of non-revelation mechanisms is rich,
which includes fairly complicated 
mechanisms. For example,
mechanisms can ask agents to reports 
both her value and prior;
or include
multiple rounds of communication 
between seller and agent who sequentially reveal
their private information.\footnote{In this model,
we assume that the buyer knows the distribution
of the sample but does not know its realization.
}
Nonetheless,
this paper designs a simple non-revelation mechanism 
--
\emph{\bidmech}\
defined as follow.
\begin{itemize}
    \item \textit{Sample-bid mechanism:}  
    Given parameter $\scale$ and sample $\sample$, 
the {\bidmech}\
solicits a non-negative bid
$\bid \geq 0$, 
allocates the item to the agent 
if $\bid \geq \sample$, 
and charges the agent $\scale \cdot \min\{\bid,\sample\}$
regardless of her allocation.
\end{itemize}
Interestingly, the \bidmech\ 
has similar format as the Becker–DeGroot–Marschak method
\citep{BDM-64}
which has been studied and implemented 
in experimental economics
for understanding agents' perception of the random event.
Here we also provide a brief comparison between
the \bidmech\ and 
the class of revelation mechanisms
in our model.
Specifically, \citet{AB-19}
show that every revelation mechanism can be characterized as a sample-based pricing defined as follows.
\begin{itemize}
 \item \textit{Sample-based pricing \citep{AB-19}:} 
    Given parameter $\scale$ and sample $\sample$, 
the sample-based pricing
solicits a non-negative bid
$\bid \geq 0$, 
allocates the item to the agent 
if $\bid \geq \alpha \sample$,
and charges the agent $\scale \sample
\cdot \mathbbm{1}\{\bid \geq \alpha \sample\}$.
\end{itemize}
It can be observed that the allocation rules
of both \bidmech\ and 
sample-based pricing are similar 
(i.e.\ competing against the sample),
and the difference is the payment semantics.

\input{Paper/table-result}

In order to beat the optimal prior-independent 
factor among revelation mechanisms, 
we need to show the approximation 
for the \bidmech\ is 
strictly better than $2$
for regular distributions,
and $\sfrac{e}{(e-1)}$ for MHR distributions.
However, approximation techniques and results for 
non-revelation mechanisms in the literature
usually contain such or even larger constants
% i.e., 2, $\sfrac{e}{e-1}$
--
for instance,
smoothness property and 
revenue covering property in
price of anarchy 
\citep[cf.][]{RST-17,har-16}.
One the other hand, analyzing the approximation 
of revelation mechanisms is relatively easier.
In 
% revelation mechanisms under 
revenue-maximization,
one analysis approach
used extensively for revelation mechanisms
is the reduction 
on revenue curves (see next paragraph).
Tight or nearly tight results have been 
built on this technique 
in both prior-independent approximation
\citep[][]{AB-18,AB-19,HJL-19}
and Bayesian approximation
\citep[][]{AHNPY-18,JLTX-19,JLQTX-19}.

Revenue curve \citep[cf.][]{BR-89}
is an equivalent representation of 
the agent's valuation distribution,
which enables clean characterizations of 
the revenue for any mechanism
\citep[see e.g.][]{mye-81,BR-89,AFHH-13}.
The high-level goal of reduction on revenue curves
is to identify a subclass of revenue curves 
% with 
% closed-form characterization 
% and 
that has closed form and 
attains the worst approximation 
guarantee.
Its main argument is 
%required 
to design 
%a reduction which modifies
a (problem or mechanism) 
specific modification on revenue curves
(i.e.\ coverts an arbitrary revenue curve 
into a revenue curve in the final subclass)
and analyze the impact of revenue
from the modification 
on the given mechanism.
Note that revenue is 
%essentially 
the
expected payment 
of the optimal bid of agent's value.
For revelation mechanisms,
after the modification has been designed,
% under revenue-maximization,
it is sufficient to study  
how payment changes for every bid
in the modification,
since 
agents are bidding truthfully 
(i.e.\ optimal bids equal their value).
However, for non-revelation mechanisms,
converting a revenue curve to another
will lead to changes in both 
the
payment for each bid and 
the 
optimal bidding strategy
of each agent.
This makes the revenue curve reduction approach
harder for non-revelation mechanisms,
and
to our knowledge, 
results of non-revelation mechanisms
in the literature
rarely
uses this technique.
In this paper, due to 
the simplicity 
of our model and the non-revelation mechanism 
considered,
we are able to apply this technique
by
% enables us to apply it in this paper by
carefully (but relatively loosely) disentangling  
these two impacts
and then analyzing them separately.

% \YF{Yingkai, can you add a small paragraph to discuss our 
% approach for the lower bound?}

In \Cref{sec:low}, we provide a lower bound on the prior-independent approximation ratio without any restriction on the family of mechanisms, 
that is, the seller can communicate with the buyer in general message space for multiple rounds. 
The crucial idea for proving the general lower bound is by observing that for pointmass distributions, 
the buyer perfectly knows the information of the seller 
and can strategically imitate the behavior of the values
in other continuous distributions. 
This prevents the seller from extracting optimal revenue from the buyer, 
which leads to a prior-independent approximation ratio at least~1.073 even with the restriction to the class of 
uniform distributions. 
This lower bound illustrates a sharp contrast to the multi-agent revenue maximization problem
where the optimal revenue can be obtained for any valuation distribution through implementation theory \citep{CR-05}.
Moreover, the general lower bound we obtained in this setting also
suggests that it is highly non-trivial to obtain the non-revelation mechanism with tight prior-independent approximation factor.

\subsection*{Important Directions}
Despite the practical impact of non-revelation mechanisms, 
the literature on mechanism design 
almost exclusively considers the design of revelation mechanisms.  
Thus, the most general direction from this paper 
is to systematically build a theory for the design of 
non-revelation mechanisms with good performance guarantee.
Some recent works on this topic are
equilibrium analysis of i.i.d.\ rank-based mechanism
\citep{CH-13}, robust analysis of welfare and revenue 
for classic mechanisms in practice (i.e.\ price of anarchy,
see discussion in the next subsection),
estimating revenue and welfare in a mechanism from equilibrium bids in another mechanism
\citep{CHN-14,CHN-16},
and the sample complexity of non-revelation mechanisms in asymmetric environments \citep{HT-19}.

Though \citet{FH-18} and this work
demonstrate non-trivial revelation gap for 
both welfare-maximization and revenue maximization,
both gaps are constant. 
Thus, one interesting open question left is to identify 
a superconstant revelation gap 
in a canonical model where 
simple non-revelation mechanisms
are sufficient to beat 
the optimal prior-independent revelation mechanisms.
As our lower bound result 
shows that no prior-independent mechanism
can achieve prior-independent approximation factor
arbitrarily close to one, 
the single-agent with single-sample access model without
any regularity assumption on distributions might be
a good candidate to answer this question.

Prior-independent mechanism design for a single item
with symmetric agents is an extensively studied model 
\citep{BK-96, FILS-15, AB-18, HJL-19}.
The fundamental difficulty is to pin down 
the optimal prior-independent approximation factor
holds even for the two-agents setting.
Recently, \citet{AB-18} obtain the tight
bounds of optimal prior-independent revelation mechanism
for MHR distributions, and 
\citet{HJL-19} generalize it to regular distributions.
In both works, the main technique is the revenue curve reduction. An open question here is to identify non-revelation 
which is simple but outperformances the optimal 
prior-independent revelation mechanism in
this single-item two-agents model.

In this work, we apply the revenue curve reduction
approach
--
a powerful technique of approximation analysis 
for revelation mechanisms
--
to a non-revelation mechanism.
Our argument is not as general as ones for 
revelation mechanisms and thus there are gaps between
the lower bound and upper bound.
Sharpening these bounds is an open question,
and may encourage more general argument 
for non-revelation mechanisms using 
the revenue curve reduction approach 
in the future work.
\subsection*{Related Work}

% \YF{Prior-independent mechanism design}
Prior-independent mechanism design, as 
a standard framework for understanding 
the robustness of mechanisms,
has been applied to 
single-dimensional mechanism design
\citep{DRY-15, RTY-12, FILS-15,AB-18, HJL-19}, multi-dimensional mechanism design 
\citep{DHKT-11,RTY-15,GK-16},
makespan minimization \citep{CHMS-13},
mechanism design for risk-averse agents 
\citep{FHH-13}, and mechanism design for agents with interdependent values \citep{CFK-14}.
Except \citet{FHH-13}, all other results 
focus on revelation mechanisms.

% \YF{Sample complexity}
There is a significant area of research studying 
mechanism design with sample access from
the distribution of agents' preference, which has two regimes -- small number of samples,
and large number of samples.
In the former regime, 
literature studies
the approximation of mechanisms with a single-sample access
\citep[e.g.][]{DRY-15, AB-19,FHL-19,DFLLR-20},
and mechanisms
with two-sample access 
\citep{BGMM-18,DZ-20}.
In the latter regime, the goal is to minimize 
the sample complexity, i.e.,
number of sample to achieve $(1 - \epsilon)$-approximation
\citep[e.g.][]{CR-14,MR-15,HMR-18,GW-18,GHZ-19,HT-19}. Except \citet{HT-19},
all other results focus on revelation mechanisms.

% \YF{Analysis for non-revelation mechanism, price of anarchy}
Price of anarchy studies how classic non-revelation mechanisms
(e.g.\ first-price auction, all-pay auction)
approximate the optimal welfare.
In \citet{ST-13}, author introduce
a smoothness property defined on mechanisms and 
give an analysis framework based on this property. 
With this smoothness framework, authors upper-bound
the welfare-approximation of the
first-price auction by $\sfrac{e}{(e-1)}$,
and 
the welfare-approximation of the all-pay auction by 2.
These two results are later improved by 
\citet{CST-15} for the all-pay auction
and \citet{HTW-18} for the first-price auction
using some mechanism-specific arguments.
\citet{HHT-14} introduce a revenue-covering
framework to analysis the price of anarchy
for both welfare and revenue.
As the instantiations of the framework,
authors upper-bound
the revenue approximation of the first-price 
auction with individual monopoly reserve 
by $\sfrac{2e}{(e-1)}$.
In all studies mentioned above, 
their results is either given by general 
analysis framework but relatively loose,
or vice versa.





==> Paper/quantile-small-old.tex <==
\subsection{Regular Distributions
with Monopoly Quantile $\monoq \leq 0.6$}

In this section, 
we first provide a method for lower bounding the revenue 
from types that bid higher than the monopoly reserve. 
Let 
\begin{align*}
\vl(\rev) = \inf_{\val} \{\val: \bid(\val, \rev) \geq \monop(\rev)\}.
\end{align*}
If $\vl(\rev) \geq \monop(\rev)$, 
then the revenue from types with value above $\vl$
is at least $\price(\vl, \rev)\cdot\quant(\vl, \rev)$.
If $\vl(\rev) < \monop(\rev)$, 
then the revenue from types with value above $\vl$
is at least 
$\price(\val, \rev)\cdot(\quant(\vl, \rev) - \monopq(\rev))
+ \price(\monop(\rev), \rev)\cdot\monopq(\rev)$.

Next we categorize the revenue curves according to their monopoly quantile, 
the quantile for value $\sfrac{\monop(\rev)}{\pscale}$,
and the expected welfare between $\monop(\rev)$ 
and $\sfrac{\monop(\rev)}{\pscale}$.
Let 
\begin{align*}
w(\rev) = \int_{\quant(\sfrac{\monop(\rev)}{\pscale}, \rev)}^{\monopq(\rev)} 
\frac{\rev(\quant)}{\quant} \dd\quant.
\end{align*}
Next lemma illustrate the method for lower bounding $\vl(\rev)$
given those parameters. 

\begin{figure}[t]
\centering
\input{Figure/critical_val_high_bid}
\caption{\label{f:critical val high bid}
Reduction for identifying critical value $\vl(\rev)$.
$\rev$ is the revenue curve for dotted line 
and $\rev'$ is the revenue curve for solid line. 
}
\end{figure}
\begin{lemma}\label{lem:critical val for high bid}
For any parameter $\quant_0 \in [0,1], \quant_1\in [0, \pscale\quant_1]$, $w\in [(1-\frac{\quant_0-\frac{\quant_1}{\pscale}}{\quant_0-\quant_1})+1-\frac{\quant_1}{\pscale\quant_0}, 
\ln(\sfrac{1}{\pscale})+1-\frac{\quant_1}{\pscale\quant_0}]$, $\val > 0$, 
if the revenue curve $\rev$ satisfies that 
$\monopq(\rev) = \quant_0$, 
$\quant(\sfrac{\monop(\rev)}{\pscale}, \rev) = \quant_1$, 
and $w(\rev) = w$, 
then the optimal bid for value $\val$ is at least $\monop(\rev)$
if for any $\quant_2 \in [\quant_0, 1]$,
letting $\bid = \min\{\sfrac{1}{\quant_2},\max\{0, \frac{\val}{\pscale}-\frac{1}{1-\quant_2}\}\}$,
$\quant_{\bid} = \frac{1}{1+\bid(1-\quant_2)}$,
we have
\begin{align*}
\val(1-\quant_1) - \quant_1\cdot\monop(\rev) - \pscale(w + \ln (\frac{\quant_2}{\quant_0}) - \frac{\ln(\quant_2)}{1-\quant_2} )
\geq \val(1-\quant_b) + \pscale\cdot \frac{\ln(\quant_{\bid})}{1-\quant_2}.
\end{align*}
\end{lemma}
\begin{proof}
Note that for any revenue curve $\rev$ illustrated in \Cref{f:critical val high bid} as the thick dotted curve, 
it is sufficient to show that the utility for bidding $\sfrac{\monop(\rev)}{\pscale}$
is higher than bidding any value below $\sfrac{\monop(\rev)}{\pscale}$.
Let $\hat{\bid}$ be the optimal bid for value $\val$.
Now suppose $\hat{\bid}$ is below $\monop$.
By \Cref{lem:revenue monotone}, 
for revenue curve $\rev'$, illustrated in \Cref{f:critical val high bid} as the solid curve, 
the optimal bid for value $\val$ is below $\hat{\val}$, 
which is lower than the monopoly reserve for $\rev'$. 
Thus it is sufficient to verify the utility for bidding $\sfrac{\monop(\rev)}{\pscale}$
is higher than bidding any value below $\sfrac{\monop(\rev)}{\pscale}$
for revenue curves that is a straight line below the monopoly reserve. 
Letting $\quant_2$ be the new lowest monopoly quantile for revenue curve $\rev'$, 
the utility for bidding $\sfrac{\monop(\rev)}{\pscale}$
is
\begin{align*}
\val(1-\quant_1) - \quant_1\cdot\monop(\rev) - \pscale(w + \ln (\frac{\quant_2}{\quant_0}) - \frac{\ln(\quant_2)}{1-\quant_2} ).
\end{align*}
Moreover, the utility for bidding any value below $\sfrac{\monop(\rev)}{\pscale}$
is at most 
\begin{align*}
\val(1-\quant_b) + \pscale\cdot \frac{\ln(\quant_{\bid})}{1-\quant_2}.
\end{align*}
where $\quant_{\bid} = \frac{1}{1+\bid(1-\quant_2)}$
and $\bid = \min\{\sfrac{1}{\quant_2},\max\{0, \frac{\val}{\pscale}-\frac{1}{1-\quant_2}\}\}$.
Note that $\bid$ is the optimal bid below $\sfrac{\monop(\rev)}{\pscale}$ is derived from the first order condition of the agent's utility as in \Cref{lem:FOC}.
Then it is sufficient to enumerate all possible value $\quant_2$
to show that the utility of bidding $\sfrac{\monop(\rev)}{\pscale}$
is higher. 
\end{proof}


The next lemma lower bounds the payment of the agent if the bid is between 0 and the monopoly reserve. 
Note that is the agent bids higher than the monopoly reserve, 
then her payment is naturally higher than the payment for bidding the monopoly reserve. 
\begin{figure}[t]
\centering
\input{Figure/rev_bid}
\caption{\label{f:rev bid}
Lower bounding the payment when the monopoly quantile is $\monopq$ and the agent bids $\bid \in [0, \sfrac{1}{\monopq}]$.
}
\end{figure}
\begin{lemma}\label{lem:rev for bid}
For any revenue curve $\rev$ with monopoly quantile $\monopq$,
for any bid $\bid \leq \sfrac{1}{\monopq}$,
the payment for bidding $\bid$ is at least 
$\pscale\cdot \frac{\ln(1+\bid(1-\monopq))}{1-\monopq}$.
% $\frac{\ln(\sfrac{1}{\quant_{\bid}})}{1-\monopq}$
% where $\quant_{\bid} = \frac{1}{1+\bid(1-\monopq)}$.
\end{lemma}
\begin{proof}
Note that the payment of the agent when she bids $\bid$ is the expected welfare truncated at $\bid$. 
The truncated welfare is minimized when the revenue curve is $\rev'$, which is a straight line for negative virtual values, as illustrated in \Cref{f:rev bid}. 
That is, we have 
\begin{equation*}
\price(\bid, \rev) \geq \price(\bid, \rev')
= \pscale\cdot (\bid\cdot\quant(\bid,\rev')
+\int_{\quant(\bid,\rev')}^1 \frac{\rev'(\quant)}{\quant} \dd\quant)
= \pscale\cdot \frac{\ln(1+\bid(1-\monopq))}{1-\monopq}.\qedhere
\end{equation*}
\end{proof}

\begin{figure}[t]
\centering
\input{Figure/quant_val}
\caption{\label{f:quant val}
Lower bounding the quantile for value $\val$.
}
\end{figure}
\begin{lemma}\label{lem:quantile for val}
For any revenue curve $\rev$ with monopoly quantile $\monopq$
and $\quant(\sfrac{\monop(\rev)}{\pscale}, \rev) = \quant_1$,
for any value $\val \leq \sfrac{1}{\monopq}$,
the quantile for value $\val$ is at least 
$\frac{1}{1+\val(1-\monopq)}$.
Moreover, for any value $\val \in [\sfrac{1}{\monopq}, \sfrac{1}{\pscale\monopq}]$,
the quantile for value $\val$ is at least 
$\frac{2\monopq-\quant_1(1+\sfrac{1}{\pscale})}{1+\val(1-\monopq)}$.
\end{lemma}
\begin{proof}
As illustrated in \Cref{f:quant val}, 
for any value $\val \leq \sfrac{1}{\pscale\monopq}$,
the quantile of the value is minimized when the revenue curve is $\rev'$, which is contains two straight lines for quantile above $\quant_1$. 
That is, for any value $\val \leq \sfrac{1}{\monopq}$, we have 
\begin{equation*}
\quant(\val, \rev) \geq \quant(\val, \rev')
= \frac{1}{1+\val(1-\monopq)}.
\end{equation*}
Moreover, for any value $\val \in [\sfrac{1}{\monopq}, \sfrac{1}{\pscale\monopq}]$,
we have 
\begin{equation*}
\quant(\val, \rev) \geq \quant(\val, \rev')
= \frac{2\monopq-\quant_1(1+\sfrac{1}{\pscale})}{1+\val(1-\monopq)}.
\qedhere
\end{equation*}
\end{proof}


By \Cref{lem:critical val for high bid},
% and \ref{lem:rev for bid}, we have that 
for any revenue curve $\rev$ that satisfies 
$\monopq(\rev) = \quant_0$, 
$\quant(\sfrac{\monop(\rev)}{\pscale}, \rev) = \quant_1$, 
and $w(\rev) = w$, 
we can lower bound the critical value $\vl(\rev)$. 
If $\vl(\rev) \geq \monop(\rev)$, 
then the revenue from types with value above $\vl$
is at least $\price(\vl, \rev)\cdot\quant(\vl, \rev)$.
Thus the revenue of the seller is 
\begin{align*}
\Rev{\rev} \geq \price(\vl, \rev)\cdot\quant(\vl, \rev) 
\geq \pscale \cdot \frac{\ln(\sfrac{1}{\quant_0})}{1-\quant_0}
\cdot \frac{2\quant_0-\quant_1(1+\sfrac{1}{\pscale})}{1+\vl(1-\quant_0)},
\end{align*}
where the last inequality holds since 
$\price(\vl, \rev) \geq  \pscale\cdot
\frac{\ln(\sfrac{1}{\quant_0})}{1-\quant_0}$
by \Cref{lem:rev for bid}, 
and $\quant(\vl, \rev) \geq \frac{2\quant_0-\quant_1(1+\sfrac{1}{\pscale})}{1+\vl(1-\quant_0)}$
by \Cref{lem:quantile for val}.
If $\vl(\rev) \leq \monop(\rev)$, 
the revenue of the seller is 
\begin{align*}
\Rev{\rev} &\geq \price(\val, \rev)\cdot(\quant(\vl, \rev) - \monopq(\rev))
+ \price(\monop(\rev), \rev)\cdot\monopq(\rev)\\
&\geq \pscale \cdot \frac{\ln(\sfrac{1}{\quant_0})}{1-\quant_0}
\cdot (\frac{1}{1+\vl(1-\quant_0)}-\quant_0)
+ \quant_0 \cdot (\frac{\quant_1}{\quant_0} + \pscale(w - \frac{\ln(\quant_0)}{1-\quant_0} )),
\end{align*}
where the last inequality holds again by invoking 
\Cref{lem:rev for bid} and \ref{lem:quantile for val}.
Therefore, to lower bound the revenue, 
it is sufficient to enumerate all possible parameters $\quant_0, \quant_1$ and $w$.

Note that the revenue lower bound we derived from the above approach is sufficient when the monopoly quantile is large. 
However, this is insufficient if the monopoly quantile is small. 
The main reason for the insufficiency is that it only calculated the revenue contribution from types with high values, 
which only occurs with small probability when the monopoly quantile is small. 
In the following lemma, we present an alternative approach for lower bounding the contribution of types with small values and small bids. 

\begin{definition}
A revenue curve $\rev$ is a \emph{pentagon} if there exists $\quant_0\in [0,1], \quant_1 \in [\quant_0, 1]$, 
such that $\rev$ is concave, 
$\rev(\quant) = 1$ for any $\quant\in [0, \quant_0]$,
and are straight lines for quantiles between $[\quant_0, \quant_1]$
and $[\quant_1, 1]$.
\end{definition}
An example of a pentagon revenue curve is illustrated as the solid curve in \Cref{f:critical bid}.


\begin{figure}[t]
\centering
\subfloat[]{
\input{Figure/critical_bid}
\label{f:critical bid a}
}
\subfloat[]{
\input{Figure/critical_bid_b}
\label{f:critical bid b}
}
\caption{\label{f:critical bid}
Lower bounding optimal bid for any value corresponding to quantile $\quant$. 
}
\end{figure}
\begin{lemma}\label{lem:lower bound bid for large quant}
For any revenue curve $\rev$ with monopoly quantile $\monopq\in [0,1]$ and any quantile $\quant\in [\monopq, 1]$, any bid $\bid \in [0, \sfrac{1}{\monopq}]$, 
if for any pentagon revenue curve $\rev'$ with parameter $\quant_0\in [\monopq, \quant], \quant_1 \in [\quant_0, 1]$, 
the optimal bid for value corresponding to $\quant$ in $\rev'$
is at least $\bid$, 
then the optimal bid for value corresponding to $\quant$ in $\rev$
is also at least $\bid$. 
\end{lemma}
\begin{proof}
For any quantile $\quant$, 
let $\hat{\bid}$ be the optimal bid for the value corresponding to quantile~$\quant$, 
and we assume that 
$\hat{\bid}$ is below monopoly reserve given revenue curve $\rev$.
If $\hat{\bid} \leq \sfrac{\rev(\quant)}{\quant}$, 
we construct the pentagon revenue curve $\rev'$ as illustrated in \Cref{f:critical bid a}. 
Note that in this case the values corresponding to quantile $\quant$ are the same for both revenue curves. 
Moreover, for this value, by \Cref{lem:revenue monotone}
its optimal bid is weaker smaller than $\hat{\bid}$ in revenue curve $\rev'$.
Thus if there exist $\bid$ such that the optimal bid for quantile $\quant$ in revenue curve $\rev'$ is above $\bid$, 
then the optimal bid $\hat{\bid}$ in revenue curve $\rev$ is also above $\bid$.
In the case $\hat{\bid} > \sfrac{\rev(\quant)}{\quant}$, 
we construct the pentagon revenue curve $\rev'$ as illustrated in \Cref{f:critical bid b}.
The only difference here is that the value corresponding to quantile $\quant$ is smaller in $\rev'$, which leads to even lower bid. 
Combining the observation, 
we can lower bound the optimal bid for any quantile by searching over pentagon revenue curves.
\end{proof}

To combine the approaches, 
for any revenue curve $\rev$, 
let $\vl$ be the critical value derived as in \Cref{lem:critical val for high bid}, 
and $\ql$ be the corresponding quantile. 
The contribution for types with quantiles smaller than $\ql$ can be bounded in the same approach. 
In addition, 
for any type with quantile larger than $\ql$, 
by \Cref{lem:lower bound bid for large quant}, 
we can calculate the lower bound on the corresponding bid $\bid(\quant)$, 
and again by \Cref{lem:rev for bid}, 
we have the lower bound on the payments for those types. 
Aggregation the contribution of the revenue provides us the desirable bound. 





% \subsection{Regular Distributions
% with Monopoly Quantile $\monoq \leq 0.4$}
% \label{sec:regular small}
% \begin{figure}[t]
% \centering
% \subfloat[]{
% \input{Figure/positive_bid}
% \label{f:show positive bid}
% }
% \subfloat[]{
% \input{Figure/lower_bound_bid}
% \label{f:minimize util difference}
% }
% \caption{\label{f:lower bound bid}
% Lower bound bid for value with small quantile.
% }
% \end{figure}


% \begin{lemma}\label{lem:lower bound bid for small quantile}
% For any distribution with monopoly quantile $\monopq < 1-\scale$
% and for any quantile $\quant \in [\monopq, 1-\scale]$, 
% the optimal bid for value with quantile $\quant$ is 
% $\bid(\quant) \geq \frac{1-\quant}{\scale\quant(1-\monopq)} - \frac{1}{1-\monopq}$. 
% \end{lemma}
% \begin{proof}
% Suppose the value with quantile $\quant$ is $\val$ 
% and the corresponding virtual value is $\virtual$. 
% We first claim that the optimal bid for value $\val$ is 
% $\bid(\val) \geq \frac{\val}{\scale} + \virtual$.
% Note that the revenue curve is concave, 
% we have $\virtual \geq -\frac{\val\quant}{1-\quant}$, 
% and hence 
% $\bid(\val) \geq \frac{\val}{\scale} - \frac{\val\quant}{1-\quant}$, 
% where the right hand side is monotone increasing in $\val$ 
% since $\frac{1}{\scale} - \frac{\quant}{1-\quant} > 0$
% for any quantile $\quant \leq 1-\scale$. 
% By the concavity of the revenue curve, 
% the value $\val \geq \frac{1-\quant}{\quant(1-\monopq)}$,
% and the optimal bid for value with quantile $\quant$ is 
% $\bid(\quant) \geq \frac{1-\quant}{\scale\quant(1-\monopq)} - \frac{1}{1-\monopq}$.


% Next we show that for value $\val$, the utility of bidding $\frac{\val}{\scale} + \virtual$
% is at least the utility for bidding $\bid \leq \val$.
% This is sufficient for the purpose of \Cref{lem:lower bound bid for small quantile}, 
% since by \Cref{lem:FOC}, 
% if bid $\bid \geq \val$, we have 
% $\bid \geq \frac{\val}{\scale} + \virtual
% \geq \frac{1-\quant}{\scale\quant(1-\monopq)} - \frac{1}{1-\monopq}$.
% Next we prove $\bid \geq \val$ by supposing in contrary the optimal bid is $\bid < \val$. 
% As illustrated in \Cref{f:lower bound bid}, 
% for revenue curve which is two straight lines with a kink, 
% the optimal bid is weakly lower than $\bid$. 
% Therefore, it is sufficient to show that for such revenue curves, 
% the optimal bid for value with quantile $\quant$ is $\bid(\quant) \geq \val$. 
% Let $\quant'\in[\monopq,1], \val'\in[0,\frac{1}{\quant'}]$ be the quantile and value corresponding to the kink of the revenue curve. 
% The optimal bid for $\bid \geq \val'$ is $\frac{\val}{\scale} + \virtual$, which is larger than $\val$ for $\quant < 1-\alpha$.
% The optimal bid for $\bid < \val'$ is 
% $\frac{\val}{\scale} - \frac{\val'\quant'}{1-\quant'}$, 
% and the utility for such bid is 
% \begin{align}\label{eq:util low bid}
% \val(1-\quant_{\bid}) + \alpha \cdot \frac{\bid\quant_{\bid}\ln \quant_{\bid}}{1-\quant_{\bid}}
% \end{align}
% where $\bid = \max\{0, \frac{\val}{\scale} - \frac{\val'\quant'}{1-\quant'}\}$
% and $\quant_{\bid} = \frac{\val'\quant'}{\val'\quant' + \bid(1-\quant')}$. 
% Note that the utility for bidding $\bid' = \frac{\val}{\scale} + \virtual$ is 
% \begin{align}\label{eq:util high bid}
% \val(1-\quant_{\bid'}) - \alpha(1-\virtual\monopq)\ln \frac{\quant'}{\quant_{\bid'}} + \frac{\alpha\val'\quant' \ln \quant'}{1-\quant'}
% \end{align}
% where $\virtual = \frac{1-\val'\quant'}{\monopq-\quant'}$ 
% and $\quant_{\bid'} = \frac{1-\virtual\monopq}{\val-\virtual}$.
% By enumerating the possible valuation for $\monopq, \val, \val', \quant'$, 
% we can verify that the utility in equation \eqref{eq:util high bid} is always higher than the utility in equation \eqref{eq:util low bid} for all desirable parameters. 
% \end{proof}


% \begin{figure}[t]
% \centering
% \input{Figure/lower_bound_bid_large_v}
% \caption{\label{f:lower bound bid large v}
% Lower bound bid for quantile smaller than monopoly quantile.
% }
% \end{figure}

% \begin{lemma}
% For any distribution with monopoly quantile $\monopq < 0.4$
% and for any quantile $\quant \in [0, \monopq]$, 
% the optimal bid for value with quantile $\quant$ is 
% $\bid(\quant) \geq \frac{1}{\monopq}$. 
% \end{lemma}
% \begin{proof}
% By \Cref{lem:monotone bid for value}, the bid of the agent is monotone in her value. 
% Thus it is sufficient to show that $\bid(\monopq) \geq \frac{1}{\monopq}$ for $\monopq < 0.4$.
% As illustrated by \Cref{f:lower bound bid large v}, 
% by \Cref{lem:revenue monotone}, 
% the bid of the agent is minimized when the revenue curve has a single kink. 
% Again it is sufficient to show that the bid of the agent with quantile at most $\min\{0.4, \monopq\}$
% is at least $\monopq$ for such revenue curves, 
% which can be verifies by numerical computation. 
% \end{proof}


% \begin{lemma}\label{lem:lower bound bid for small quantile case 2}
% For any distribution with monopoly quantile $\monopq < 0.4$
% and for any quantile $\quant \in [\monopq, 0.4]$, 
% the optimal bid for value with quantile $\quant$ is 
% $\bid(\quant) \geq $. 
% \end{lemma}

==> intro.tex <==
\section{Goal}

In this project,
we want to study 
the revelation gap for sample based pricing. 
In this setting, the seller has a single item to sell,
and the seller only has a sample to infer the distribution of the buyer. 
If the sample is the value sample, 
then this is the classical model studied in \citet{AB-19}, 
and we want to show that there is a constant gap 
between the optimal revelation mechanism and the optimal non-revelation mechanism. 
If the sample is the sample from the bid space, 
then in some cases this is equivalent to the mechanism design for digital good environment when there are two buyers. 
We assume the prior distribution is regular or MHR. 



